Efficient Numerical Wave Propagation Enhanced By An End-to-End Deep Learning Model

In a variety of scientific and engineering domains, the need for high-fidelity and efficient solutions for high-frequency wave propagation holds great significance. Recent advances in wave modeling use sufficiently accurate fine solver outputs to train a neural network that enhances the accuracy of a fast but inaccurate coarse solver. In this paper we build upon the work of Nguyen and Tsai (2023) and present a novel unified system that integrates a numerical solver with a deep learning component into an end-to-end framework. In the proposed setting, we investigate refinements to the network architecture and data generation algorithm. A stable and fast solver further allows the use of Parareal, a parallel-in-time algorithm to correct high-frequency wave components. Our results show that the cohesive structure improves performance without sacrificing speed, and demonstrate the importance of temporal dynamics, as well as Parareal, for accurate wave propagation.

==> chapters/2.related_work.tex <==
\section{Related Work}\label{ch:related-work}




==> figures/data_generation.tex <==
\begin{tikzpicture}
    [
  rednode/.style={shape=rectangle, draw=red, line width=1},
  bluenode/.style={shape=rectangle, draw=blue, line width=1},
]

    \tikzstyle{every node}=[font = \large]

    \rmfamily
    \draw[->] (0,.6) -- (13,.6) node[below] {\large \hspace{-13mm} network use};
    \draw[->] (.5,.3) -- (.5,8.5) node[left] {\large time};

    \node[draw=blue] at (2, .3) {$u_0$};
    \node[draw=blue] at (2, 2) {$y_1$};
    \node[draw=red] at (4, 2) {$x_1^1$};

    \node[draw=blue] at (2,3.4) {$y_2$};
    \node[draw=red] at (4, 3.4) {$x_2^1$};
    \node[draw=red] at (6, 3.4) {$x_2^2$};
    \node[draw=blue] at (2,4.8) {$y_3$};
    \node[draw=red] at (4, 4.8) {$x_3^1$};
    \node[draw=red] at (6, 4.8) {$x_3^2$};
    \node[draw=red] at (8, 4.8) {$x_3^3$};
    \node[draw=blue] at (2,6.2) {$y_4$};
    \node[draw=red] at (4, 6.2) {$x_4^1$};
    \node[draw=red] at (6, 6.2) {$x_4^2$};
    \node[draw=red] at (8, 6.2) {$x_4^3$};
    \node[draw=red] at (10, 6.2) {$x_4^4$};
    \node[draw=blue] at (2,7.6) {$y_5$};
    \node[draw=red] at (4, 7.6) {$x_5^1$};
    \node[draw=red] at (6, 7.6) {$x_5^2$};
    \node[draw=red] at (8, 7.6) {$x_5^3$};
    \node[draw=red] at (10, 7.6) {$x_5^4$};
    \node[draw=red] at (12, 7.6) {$x_5^5$};


    \draw[->] (2,.7) -- (2,1.75) node[left, midway] {$\mathcal{F}_{\Delta t}$};
    \draw[->] (2,2.25) -- (2,3.15) node[left, midway] {$\mathcal{F}_{\Delta t}$};
    \draw[->] (2,3.65) -- (2,4.55) node[left, midway] {$\mathcal{F}_{\Delta t}$};
    \draw[->] (2,5.05) -- (2,5.95) node[left, midway] {$\mathcal{F}_{\Delta t}$};
    \draw[->] (2,6.45) -- (2,7.35) node[left, midway] {$\mathcal{F}_{\Delta t}$};
    \draw[dashed, ->] (2.25+.15,.71+.15) -- (3.63,1.7) node[below, midway] {\hspace{4mm}$\Psi_{\Delta t}^\theta$};
    \draw[dashed, ->] (4.45,2.25) -- (5.63,3.1) node[below, midway] {\hspace{4mm}$\Psi_{\Delta t}^\theta$};
    \draw[dashed, ->] (6.45,3.65) -- (7.63,4.5) node[below, midway] {\hspace{4mm}$\Psi_{\Delta t}^\theta$};
    \draw[dashed, ->] (8.45,5.05) -- (9.63,5.9) node[below, midway] {\hspace{4mm}$\Psi_{\Delta t}^\theta$};
    \draw[dashed, ->] (10.45,6.45) -- (11.63,7.3) node[below, midway] {\hspace{4mm}$\Psi_{\Delta t}^\theta$};
    \draw[dashed, ->] (2.25+.15,2.11+.15) -- (3.63,3.1) node[below, midway] {};
    \draw[dashed, ->] (2.25+.15,3.51+.15) -- (3.63,4.5) node[below, midway] {};
    \draw[dashed, ->] (2.25+.15,4.91+.15) -- (3.63,5.9) node[below, midway] {};
    \draw[dashed, ->] (2.25+.15,6.31+.15) -- (3.63,7.3) node[right, midway] {};
    \draw[dashed, ->] (4.45,3.65) -- (5.63,4.5) node[right, midway] {};
    \draw[dashed, ->] (4.45,5.05) -- (5.63,5.9) node[right, midway] {};
    \draw[dashed, ->] (4.45,6.45) -- (5.63,7.3) node[right, midway] {};
    \draw[dashed, ->] (6.45,5.05) -- (7.63,5.9) node[right, midway] {};
    \draw[dashed, ->] (6.45,6.45) -- (7.63,7.3) node[right, midway] {};
    \draw[dashed, ->] (8.45,6.45) -- (9.63,7.3) node[right, midway] {};


    \node[draw, below left] at (12.5,3) {
        \begin{tabular}{cl}
            \begin{tikzpicture}
                \node [rednode] {};
            \end{tikzpicture} & outputs ($\Psi_{\Delta t}^\theta$)\\
            \begin{tikzpicture}
                \node [bluenode] {};
            \end{tikzpicture} & labels ($\mathcal{F}_{\Delta t}$)\\
            \begin{tikzpicture}
                \path[->, black] (0, -.1) edge (0.4, -.1);
                \path[dashed, ->, black] (0, .1) edge (0.4, .1);
            \end{tikzpicture} & iteration $\Delta t$ \\
        \end{tabular}
    };

\end{tikzpicture}
